Ocassionally Secure: A Comparative Analysis of Code Generation Assistants

$ $Large Language Models (LLMs) are being increasingly utilized in various applications, with code generations being a notable example. While previous research has shown that LLMs have the capability to generate both secure and insecure code, the literature does not take into account what factors help generate secure and effective code. Therefore in this paper we focus on identifying and understanding the conditions and contexts in which LLMs can be effectively and safely deployed in real-world scenarios to generate quality code. We conducted a comparative analysis of four advanced LLMs--GPT-3.5 and GPT-4 using ChatGPT and Bard and Gemini from Google--using 9 separate tasks to assess each model's code generation capabilities. We contextualized our study to represent the typical use cases of a real-life developer employing LLMs for everyday tasks as work. Additionally, we place an emphasis on security awareness which is represented through the use of two distinct versions of our developer persona. In total, we collected 61 code outputs and analyzed them across several aspects: functionality, security, performance, complexity, and reliability. These insights are crucial for understanding the models' capabilities and limitations, guiding future development and practical applications in the field of automated code generation.

==> conclusion.tex <==
%!TEX root=paper.tex

\section{Conclusion}
\label{sec:conclusion}
%Large Language Models (LLMs) are gaining widespread use in automating various software development tasks, with code generation being a notable application. In this study, we delve into the diverse code outputs generated by different LLMs when exposed to identical prompts and tasks. Our comparative analysis focuses on four prominent LLMs: GPT-3.5 and GPT-4 within ChatGPT, and Google's Bard and Gemini. The goal is to unveil the factors influencing variations in code quality and efficiency across these models. Importantly, our analysis serves as a guide for developers, shedding light on best practices and practical realities when leveraging these LLMs in code generation workflows.
%
%Our research makes three significant contributions to the field of code generation using Large Language Models (LLMs). Firstly, we identified a lack of consistency in the code generated by different LLMs. This inconsistency manifests in the variations in code structure and functionality, indicating a model-dependent variability in code generation.
%Secondly, our comprehensive analysis, encompassing both manual and automated security reviews, revealed that the security of generated code is also inconsistent. Notably, similar code segments intended for different applications exhibited disparate levels of security robustness. The most prevalent security concerns identified were related to input validation, sanitization, and secret key management. This finding highlights the necessity for users employing LLMs for code generation to remain vigilant regarding these specific security vulnerabilities.
%
%Lastly, our investigation into the impact of personas on the output code quality revealed interesting effects across different language models. Notably, when employing the security persona with GPT-3.5, GPT-4, and Bard, we observed a reduction in the number of security vulnerabilities compared to using the normal persona. However, the opposite trend was noticed with Gemini, where the use of the security persona resulted in an increase in security vulnerabilities. In terms of functionality, the influence of personas on the models' outputs was less evident. 

